Flares in Open Clusters with K2. II. Pleiades, Hyades, Praesepe, Ruprecht 147, and M67

Flares, energetic eruptions on the surfaces of stars, are an unmistakable manifestation of magnetically driven emission. Their occurrence rates and energy distributions trace stellar characteristics such as mass and age. But before flares can be used to constrain stellar properties, the flaring-age-mass relation requires proper calibration. This work sets out to quantify flaring activity of independently age-dated main sequence stars for a broad range of spectral types using optical light curves obtained by the Kepler satellite. Drawing from the complete K2 archive, we searched 3435 $\sim 80$ day long light curves of 2111 open cluster members for flares using the open-source software packages K2SC to remove instrumental and astrophysical variability from K2 light curves, and AltaiPony to search and characterize the flare candidates. We confirmed a total of 3844 flares on high probability open cluster members with ages from zero age main sequence (Pleiades) to 3.6 Gyr (M67). We extended the mass range probed in the first study of this series to span from Sun-like stars to mid-M dwarfs. We added the Hyades (690 Myr) to the sample as a comparison cluster to Praesepe (750 Myr), the 2.6 Gyr old Ruprecht 147, and several hundred light curves from the late K2 Campaigns in the remaining clusters. The flare energy distribution was similar in the entire parameter space, following a power law relation with exponent $\alpha\approx 1.84-2.39$. The flaring rates declined with age, and declined faster for higher mass stars. We found evidence that a rapid decline in flaring activity occurred in M1-M2 dwarfs around Hyades/Praesepe age, when these stars spun down to rotation periods of about 10 days, while higher mass stars had already transitioned to lower flaring rates, and lower mass stars still resided in the saturated activity regime. (abridged)

==> tables/powerlaw_fullsample_wheatland.tex <==
\begin{tabular}{lccr}
\hline\hline
  &                               $ED$ &                                  $E_\mathrm{Kp}$ \\
\hline
$\alpha$            &  $2.10\left(^{0.04}_{0.04}\right)$ &                $1.98\left(^{0.03}_{0.03}\right)$ \\
$\beta$ [yr$^{-1}$] &    $2023\left(^{600}_{460}\right)$ &  $4.01\left(^{32.15}_{3.55}\right)\cdot 10^{32}$ \\
$n_\mathrm{tot}$    &                               3844 &                                             3844 \\
$n_\mathrm{fit}$    &                                961 &                                             1213 \\
min.                &                              629 s &                          $6.63\cdot 10^{32}$ erg \\
max.                &                            82185 s &                          $3.01\cdot 10^{35}$ erg \\
\hline

\end{tabular}


==> tables/powerlaw_literature.tex <==

\begin{tabular}{lL{6cm}L{4cm}l}
%ONLY COPY BELOW THIS LINE
\hline\hline
                      Who &                                                                                  method &                                                          data &      $\alpha-1$ \\
\hline
  Hawley et al. (2014)    &    LSq with Poisson uncertainty, increase the low energy limit until the fit is robust  &                                                               &     .95 (binned), 1.01 (cumulative)      \\
  Davenport (2016)        &            weighted LSq, asymmetric Poisson confidence intervals following Gehrels1986  &                                                               &                 \\
  Gizis  (2017)           &    de-biased MLE (Arnold2015), weight each point with sqrt(N) in each bin (Clauset+2009 &                                                              22 flares on one M7 UCD &   .6-1. (31-33 erg)              \\
  Paudel et al. (2018)    &                               ML from a paper in 2010, used emcee (Foreman-Mackey2013)  &                                                               &                 \\
  Lacy (1976)             &                                                                  graphical, linear LSq  &                                        386 flares on UV Cetis &         .43-1.  \\
  Güdel et al.(2003)      &      -                                                                                   &                                                               &                 \\
  Davenport et al. (2012) &              Fit $\log_{10} Y = \alpha + (\beta \log_{10} X)(10 -\gamma /(X+\delta) )$  &  $\sim$50,000 M dwarfs from SDSS and 1321 M dwarfs from 2MASS &          .9-2.1 \\
  Lurie et al. (2015)     &   Bayesian Markov chain Monte Carlo based algorithm (Kelly 2007) for linear regression  &                                                2 dMe5 dwarfs  &        .92-1.03 \\
  Audard et al. (2000)    &                                                      Crawford+1970 MLE (Jauncey-style)  &                    EUVE 12 F-M type stars, 10-20 flares each  &        .46-1.61 \\
  Shakhovskaia (1989)     &                      linear representation, power laws from Gershberg/Shakhovskaya1983  &                                     30-40 dK0-dM8, 200 flares &          .4-1.4 \\
  Yang et al. (2017)      &                                                                            binned FFDs  &                 103187 flares on 540 M-type dwarfs in Kepler  &   1.07 +/- 0.35 \\
  Howard et al. (2018)    & fit a cumulative power law, MCMC for uncertainties &575 flares on 284 stars & 0.84-1.34\\
  Hilton et al. (2011) &&&.63-.83\\ 
\bottomrule
\end{tabular}

